Control Synthesis of Nonlinear Sampled Switched Systems using Euler's Method

In this paper, we propose a symbolic control synthesis method for nonlinear sampled switched systems whose vector fields are one-sided Lipschitz. The main idea is to use an approximate model obtained from the forward Euler method to build a guaranteed control. The benefit of this method is that the error introduced by symbolic modeling is bounded by choosing suitable time and space discretizations. The method is implemented in the interpreted language Octave. Several examples of the literature are performed and the results are compared with results obtained with a previous method based on the Runge-Kutta integration method.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{E. {\'A}brah{\'a}m and S. Bogomolov (Eds.): 3rd International\\ Workshop on Symbolic and Numerical Methods for Reachability\\ Analysis (SNR 2017)\\
EPTCS 247, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.247.2}{10.4204/EPTCS.247.2}}
\pdfoutput=1

